Automatic Discovery of Visual Circuits

To date, most discoveries of network subcomponents that implement human-interpretable computations in deep vision models have involved close study of single units and large amounts of human labor. We explore scalable methods for extracting the subgraph of a vision model's computational graph that underlies recognition of a specific visual concept. We introduce a new method for identifying these subgraphs: specifying a visual concept using a few examples, and then tracing the interdependence of neuron activations across layers, or their functional connectivity. We find that our approach extracts circuits that causally affect model output, and that editing these circuits can defend large pretrained models from adversarial attacks.

==> latex/02_related.tex <==
\section{Related Work}
\label{sec:related}

\textbf{Attributing Model Behavior: } Approaches such as saliency mapping attempt to form explanations for how neural networks respond to inputs by highlighting the regions of images that have the strongest effect on model predictions. However, such methods frequently propose

\textbf{Automated Circuit Extraction: } Various approaches have attempted to find circuits in neural networks both manually and automatically. A significant amount of recent work has focused on finding circuits that execute specific functions in language models, such as indirect object identification~\cite{wang2022interpretability}. More recently, this form of circuit detection can be automated by algorithms such as ACDC by Conmy et al.~\cite{conmy2023automated}. Motivated by the promise of this approach and the need for [scalable circuit detection], our work provides TODO. 

In vision models, there has been some manual exploration of circuits by analyzing feature visualizations and mnanually aggregating weights by Olah et al.~\cite{olah2020zoom}, as well as exploration of automatically finding subnetworks of neurons that activate highly on specific visual concepts, such as Hohman et al.~\cite{hohman2019summit}. We extend from this work by proposing a new model of automatically finding circuits for visual features. 

\textbf{Model Editing/Steering: } Interpretability work often stops at attempting to give explanations of a model's behavior, but this increases considerably in utility if it can be used to steer a model toward desired outcome. For example, Meng et al.~\cite{meng2022locating} show that models can be edited to add factual information. 
